A Theoretical Analysis of Joint Manifolds

The emergence of low-cost sensor architectures for diverse modalities has made it possible to deploy sensor arrays that capture a single event from a large number of vantage points and using multiple modalities. In many scenarios, these sensors acquire very high-dimensional data such as audio signals, images, and video. To cope with such high-dimensional data, we typically rely on low-dimensional models. Manifold models provide a particularly powerful model that captures the structure of high-dimensional data when it is governed by a low-dimensional set of parameters. However, these models do not typically take into account dependencies among multiple sensors. We thus propose a new joint manifold framework for data ensembles that exploits such dependencies. We show that simple algorithms can exploit the joint manifold structure to improve their performance on standard signal processing applications. Additionally, recent results concerning dimensionality reduction for manifolds enable us to formulate a network-scalable data compression scheme that uses random projections of the sensed data. This scheme efficiently fuses the data from all sensors through the addition of such projections, regardless of the data modalities and dimensions.

==> jam2.tex <==
\section{Joint manifolds}
\label{sec:jam}

In this section we develop a theoretical framework for ensembles of
manifolds which are {\em jointly} parameterized by a small number of
{\em common} degrees of freedom. Informally, we propose a data
structure for jointly modeling such ensembles; this is obtained by
concatenating points from different ensembles that are indexed by
the same articulation parameter to obtain a single point in a
higher-dimensional space. We begin by defining the joint manifold
for the general setting of arbitrary topological manifolds\footnote{A comprehensive introduction of topological manifolds can be found in Boothby~\cite{Boothby}.}.

\begin{definition}
Let $\manifold_1,\manifold_2,\ldots,\manifold_J$ be an ensemble of
$J$ topological manifolds of equal dimension $K$.  Suppose that the
manifolds are homeomorphic to each other, in which case there exists
a homeomorphism $\psi_{j}$ between $\manifold_1$ and $\manifold_j$
for each $j$.  For a particular set of mappings $\{ \psi_j
\}_{j=2}^J$, we define the {\bf joint manifold} as
$$
\manifold^* = \{(p_1,p_2,\ldots,p_J) \in \manifold_1 \times
\manifold_2 \times \cdots \times \manifold_J : p_j = \psi_j(p_1), 2
\le j \le J \}.
$$
Furthermore, we say that
$\manifold_1,\manifold_2,\ldots,\manifold_J$ are the corresponding
{\bf component manifolds}.
\end{definition}

Notice that $\manifold_1$ serves as a common {\em parameter space}
for all the component manifolds.  Since the component manifolds are
homeomorphic to each other, this choice is ultimately arbitrary.  In
practice it may be more natural to think of each component manifold
as being homeomorphic to some fixed $K-$dimensional parameter space $\Theta$.
%, which is
%{\em not} one of the manifolds used to construct $\manifold^*$.
However, in this case one could still define $\manifold^*$ as is
done above by defining $\psi_j$ as the composition of the
homeomorphic mappings from $\manifold_1$ to $\Theta$ and from
$\Theta$ to $\manifold_j$.

As an example, consider the one-dimensional manifolds in Figure
\ref{fig:helix}.  Figures \ref{fig:helix} (a) and (b) show two
isomorphic manifolds, where $\manifold_1 = (0, 2\pi)$ is an open
interval, and $\manifold_2 = \{ \psi_2(\theta) : \theta \in
\manifold_1 \}$ where $\psi_2(\theta) = (\cos(\theta),
\sin(\theta))$, i.e., $\manifold_2 = S^1 \backslash (1,0)$ is a
circle with one point removed (so that it remains isomorphic to a
line segment).  In this case the joint manifold $\manifold^* = \{
(\theta, \cos(\theta), \sin(\theta)) : \theta \in (0,2\pi) \}$,
illustrated in Figure \ref{fig:helix} (c), is a helix.  Notice that
there exist other possible homeomorphic mappings from $\manifold_1$
to $\manifold_2$, and that the precise structure of the joint
manifold as a submanifold of $\reals^3$ is heavily dependent on the
choice of this mapping.

\begin{figure}[!t]
\centering
\begin{tabular}{ccc}
{\includegraphics[width=0.3\hsize]{Figs/line}} &
{\includegraphics[width=0.3\hsize]{Figs/circle}} &
{\includegraphics[width=0.4\hsize, viewport=50 60 400 300]{Figs/helix}} \\
(a) $\manifold_1 \subseteq \reals$: line segment & (b) $\manifold_2 \subseteq \reals^2$:
circle segment & (c) $\manifold^* \subseteq \reals^3$: helix segment
\end{tabular}
\caption{\small\sl A pair of isomorphic manifolds $\manifold_1$ and
$\manifold_2$, and the resulting joint manifold $\manifold^*$.}
\label{fig:helix}
\end{figure}

Returning to the definition of $\manifold^*$, observe that although
we have called $\manifold^*$ the joint manifold, we have not shown
that it actually forms a topological manifold. To prove that
$\manifold^*$ is indeed a manifold, we will make use of the fact
that the joint manifold is a subset of the {\em product manifold}
$\manifold_1 \times \manifold_2 \times \cdots \times \manifold_J$.
One can show that the product manifold forms a $JK$-dimensional manifold
using the product topology~\cite{Boothby}. By comparison, we now
show that $\manifold^*$ has dimension only $K$.

\begin{prop} \label{prop:manifold}
$\manifold^*$ is a $K$-dimensional submanifold of $\manifold_1
\times \manifold_2 \times \cdots \times \manifold_J$.
\end{prop}
\begin{proof}
We first observe that since $\manifold^*$ is a subset of the product
manifold, we automatically have that $\manifold^*$ is a second
countable Hausdorff topological space.  Thus, all that remains is to
show that $\manifold^*$ is locally homeomorphic to $\reals^K$.  Let
$p = (p_1, p_2, \ldots, p_J)$ be an arbitrary point on
$\manifold^*$.  Since $p_1 \in \manifold_1$, we have a pair $(U_1,
\phi_1)$ such that $U_1 \subset \manifold_1$ is an open set
containing $p_1$ and $\phi_1 : U_1 \rightarrow V$ is a homeomorphism
where $V$ is an open set in $\reals^K$.  We now define for $2 \le j \le J$ $U_j =
\psi_j(U_1)$ and $\phi_j = \phi_1 \circ \psi_j^{-1} : U_j
\rightarrow V$.  Note that for each $j$, $U_j$ is an open set and
$\phi_j$ is a homeomorphism (since $\psi_j$ is a homeomorphism).

Now define $U^* = (U_1 \times U_2 \times \cdots \times U_J) \cap
\manifold^*$.  Observe that $U^*$ is an open set and that $p \in
U^*$.  Furthermore, let $q = (q_1,q_2, \ldots, q_J)$ be any element
of $U^*$. Then $\phi_j(q_j) = \phi_1 \circ \psi_j^{-1}(q_j) = \phi_1
(q_1)$ for each $2 \le j \le J$. Thus, since the image of each $q_j
\in U_j$ in $V$ under their corresponding $\phi_j$ is the same, we
can form a single homeomorphism $\phi^*: U^* \to V$ by assigning
$\phi^*(q) = \phi_1(q_1)$. This shows that $\manifold^*$ is locally
homeomorphic to $\reals^K$ as desired.
\end{proof}

Since $\manifold^*$ is a submanifold of $\manifold_1 \times
\manifold_2 \times \cdots \times \manifold_J$, it also inherits some
desirable properties from its component manifolds.

\begin{prop}
Suppose that $\manifold_1, \manifold_2, \ldots \manifold_J$ are
isomorphic topological manifolds and $\manifold^*$ is defined as
above.
\begin{enumerate}
%\item If $\manifold_1, \manifold_2, \ldots, \manifold_J$ are smooth,
%then $\manifold^*$ is smooth.
\item If $\manifold_1, \manifold_2, \ldots, \manifold_J$ are Riemannian,
then $\manifold^*$ is Riemannian.
\item If $\manifold_1, \manifold_2, \ldots, \manifold_J$ are compact,
then $\manifold^*$ is compact.
\end{enumerate}
\end{prop}
\begin{proof}
The proofs of these facts are straightforward and follow from the
fact that if the component manifolds are Riemannian or compact, then
the product manifold will be as well.  $\manifold^*$ then inherits
these properties as a submanifold of the product
manifold~\cite{Boothby}.
\end{proof}

Up to this point we have considered general topological manifolds.
In particular, we have {\em not} assumed that the component
manifolds are embedded in any particular space.  If each component
manifold $\manifold_j$ is embedded in $\reals^{N_j}$, the joint
manifold is naturally embedded in $\reals^{N^*}$ where $N^* =
\sum_{j=1}^J N_j$. Hence, the joint manifold can be viewed as a
model for data of {\em varying ambient dimension} linked by a common
parametrization.  In the sequel, we assume that each manifold
$\manifold_j$ is embedded in $\reals^N$, which implies that
$\manifold^* \subset \reals^{JN}$. Observe that while the intrinsic
dimension of the joint manifold remains constant at $K$, the ambient
dimension increases by a factor of $J$.  We now examine how a number
of geometric properties of the joint manifold compare to those of
the component manifolds.

We begin with the following simple observation that Euclidean
distances between points on the joint manifold are larger than
distances on the component manifolds.  In the remainder of this
paper, whenever we use the notation $\| \cdot \|$ we mean $\| \cdot
\|_{\ell_2}$, i.e., the $\ell_2$ (Euclidean) norm on $\reals^N$.
When we wish to differentiate this from other $\ell_p$ norms, we
will be explicit.

\begin{prop} \label{prop:euclidean}
Let $p = (p_1, p_2, \ldots, p_J)$ and $q = (q_1, q_2, \ldots, q_J)$
be two points on the joint manifold $\manifold^*$.  Then
$$
\|p-q\| = \sqrt{\sum_{j=1}^J \|p_j-q_j\|^2}.
$$
\end{prop}
\begin{proof}
This follows from the definition of the Euclidean norm:
$$
\|p-q\|^2 = \sum_{i=1}^{JN} (p(i)-q(i))^2 = \sum_{j=1}^J
\sum_{i=1}^N (p_j(i) - q_j(i))^2 = \sum_{j=1}^J \|p_j - q_j\|^2.
$$
\end{proof}

While Euclidean distances are important (especially when noise is
introduced), the natural measure of distance between a pair of
points on a Riemannian manifold is not Euclidean distance, but
rather the {\em geodesic distance}.  The geodesic distance between
points $p,q \in \manifold$ is defined as
\begin{equation} \label{eq:geodesic}
d_\manifold(p,q) = \inf \{ L(\gamma) : \gamma(0) = p, \gamma(1) = q
\},
\end{equation}
where $\gamma : [0,1] \rightarrow \manifold$ is a $C^1$-smooth curve
joining $p$ and $q$, and $L(\gamma)$ is the length of $\gamma$ as
measured by
\begin{equation}
L(\gamma) = \int_0^1 \|\dot{\gamma}(t)\| dt.
\end{equation}
In order to see how geodesic distances on $\manifold^*$ compare to
geodesic distances on the component manifolds, we will make use of
the following lemma.

\begin{lemma} \label{lemma:paths}
Suppose that $\manifold_1, \manifold_2, \ldots, \manifold_J$ are
Riemannian manifolds, and let $\gamma : [0,1] \rightarrow
\manifold^*$ be a $C^1$-smooth curve on the joint manifold.  Then we
can write $\gamma = (\gamma_1, \gamma_2, \ldots, \gamma_J)$ where
each $\gamma_j : [0,1] \rightarrow \manifold_j$ is a $C^1$-smooth
curve on $\manifold_j$, and
$$
\frac{1}{\sqrt{J}} \sum_{j=1}^J L(\gamma_j) \le L(\gamma) \le
\sum_{j=1}^J L(\gamma_j).
$$
\end{lemma}
\begin{proof}
We begin by observing that
\begin{equation} \label{eq:paths1}
L(\gamma) = \int_0^1 \|\dot{\gamma}(t)\| dt = \int_0^1 \sqrt{
\sum_{j=1}^J \|\dot{\gamma_j}(t)\|^2} \ dt.
\end{equation}
For a fixed $t$, let $x_j = \|\dot{\gamma_j}(t)\|$, and observe that
$(x_1, x_2, \ldots, x_J)$ is a vector in $\reals^J$.  Thus we may
apply the standard norm inequalities
\begin{equation} \label{eq:normiq}
\frac{1}{\sqrt{J}} \|x\|_{\ell_1} \le \|x\|_{\ell_2} \le
\|x\|_{\ell_1}
\end{equation}
to obtain
\begin{equation} \label{eq:paths2}
\frac{1}{\sqrt{J}} \sum_{j=1}^J \|\dot{\gamma_j}(t)\| \le \sqrt{
\sum_{j=1}^J \|\dot{\gamma_j}(t)\|^2} \le \sum_{j=1}^J
\|\dot{\gamma_j}(t)\|.
\end{equation}
Combining the right-hand side of (\ref{eq:paths2}) with
(\ref{eq:paths1}) we obtain
$$
L(\gamma) \le \int_0^1 \sum_{j=1}^J \|\dot{\gamma_j}(t)\| dt =
 \sum_{j=1}^J \int_0^1 \|\dot{\gamma_j}(t)\| dt = \sum_{j=1}^J
 L(\gamma_j).
$$
Similarly, from the left-hand side of (\ref{eq:paths2}) we obtain
$$
L(\gamma) \ge \int_0^1 \frac{1}{\sqrt{J}} \sum_{j=1}^J
\|\dot{\gamma_j}(t)\| dt = \frac{1}{\sqrt{J}}
 \sum_{j=1}^J \int_0^1 \|\dot{\gamma_j}(t)\| dt = \frac{1}{\sqrt{J}} \sum_{j=1}^J
 L(\gamma_j).
$$
\end{proof}

We are now in a position to compare geodesic distances on
$\manifold^*$ to those on the component manifold.

\begin{thm} \label{thm:geod}
Suppose that $\manifold_1, \manifold_2, \ldots, \manifold_J$ are
Riemannian manifolds. Let $p = (p_1, p_2, \ldots, p_J)$ and $q =
(q_1, q_2, \ldots, q_J)$ be two points on the corresponding joint manifold
$\manifold^*$.  Then
\begin{equation} \label{eq:geod1}
d_{\manifold^*}(p,q) \ge \frac{1}{\sqrt{J}} \sum_{j=1}^J
d_{\manifold_j}(p_j,q_j).
\end{equation}
If the mappings $\psi_2, \psi_3, \ldots, \psi_J$ are {\em
isometries}, i.e., $d_{\manifold_1}(p_1,q_1) =
d_{\manifold_j}(\psi_j(p_1),\psi_j(q_1))$ for any $j$ and for any
pair of points ($p,q$), then
\begin{equation} \label{eq:geod2}
d_{\manifold^*}(p,q) = \frac{1}{\sqrt{J}} \sum_{j=1}^J
d_{\manifold_j}(p_j,q_j) = \sqrt{J} \cdot d_{\manifold_1}(p_1,q_1).
\end{equation}
\end{thm}
\begin{proof}
If $\gamma$ is a geodesic path between
$p$ and $q$, then from Lemma \ref{lemma:paths},
$$
d_{\manifold^*}(p,q) = L(\gamma) \ge \frac{1}{\sqrt{J}} \sum_{j=1}^J
L(\gamma_j).
$$
By definition $L(\gamma_j) \ge d_{\manifold_j}(p_j,
q_j)$; hence, this establishes (\ref{eq:geod1}).

Now observe that lower bound in Lemma \ref{lemma:paths} is derived
from the lower inequality of (\ref{eq:normiq}).  This inequality is
attained with equality if and only if each term in the sum is equal,
i.e., $L(\gamma_j) = L(\gamma_k)$ for all $j$ and $k$. This is
precisely the case when $\psi_2, \psi_3, \ldots, \psi_J$ are
isometries.  Thus we obtain
$$
d_{\manifold^*}(p,q) = L(\gamma) = \frac{1}{\sqrt{J}} \sum_{j=1}^J
L(\gamma_j) = \sqrt{J} L(\gamma_1).
$$
We now conclude that $L(\gamma_1) = d_{\manifold_1}(p_1,q_1)$ since
if we could obtain a shorter path $\tilde{\gamma_1}$ from $p_1$ to
$q_1$ this would contradict the assumption that $\gamma$ is a
geodesic on $\manifold^*$, which establishes (\ref{eq:geod2}).
\end{proof}

Next, we study local smoothness and global self avoidance properties
of the joint manifold using the notion of {\em condition number}.

\begin{definition}{\em \cite{niyogi}}
Let $\manifold$ be a Riemannian submanifold of $\reals^\dim$. The
{\bf condition number} is defined as $1/\condition$, where
$\condition$ is the largest number satisfying the following: the
open normal bundle about $\manifold$ of radius $r$ is embedded in
$\reals^\dim$ for all $r < \condition$.
\end{definition}

\begin{comment}The condition number is closely related to classically studied
properties of manifolds such as curvature and the second fundamental
form. For instance, $1/\tau$ serves as an upper bound for the
absolute value of the second derivative of any $C^2$-curve on a
smooth manifold.
\end{comment}

The condition number of a given manifold controls both local
smoothness properties and global properties of the manifold.
Intuitively, as $1/\tau$ becomes smaller, the manifold becomes
smoother and more self-avoiding.  This is made more precise in the
following lemmata.

\begin{lemma}{\em \cite{niyogi}}
Suppose $\manifold$ has condition number $1/\tau$.  Let $p,q \in
\manifold$ be two distinct points on $\manifold$, and let
$\gamma(t)$ denote a unit speed parameterization of the geodesic
path joining $p$ and $q$.  Then
$$
\max_t \|\ddot{\gamma}(t)\| \le \frac{1}{\tau}.
$$
\end{lemma}

\begin{lemma}{\em \cite{niyogi}} \label{lem:cond_geodesics}
Suppose $\manifold$ has condition number $1/\tau$.  Let $p,q \in
\manifold$ be two points on $\manifold$ such that $\|p-q\| = d.$  If
$d \le \tau/2$, then the geodesic distance $d_\manifold(p,q)$ is
bounded by
$$
d_\manifold(p,q) \le \tau (1 - \sqrt{1 - 2d/\tau}).
$$
\end{lemma}

We wish to show that if the component manifolds are smooth and self
avoiding, the joint manifold is as well. It is not easy to prove
this in the most general case, where the only assumption is that
there exists a homeomorphism (i.e., a continuous bijective map
$\psi$) between every pair of manifolds. However, suppose the
manifolds are {\em diffeomorphic}, i.e., there exists a continuous
bijective map between tangent spaces at corresponding points on
every pair of manifolds. In that case, we make the following assertion.
\begin{thm} \label{thm:cond_jam}
Suppose that $\manifold_1, \manifold_2, \ldots, \manifold_J$ are
Riemannian submanifolds of $\reals^N$, and let $1/\tau_j$ denote the
condition number of $\manifold_j$. Suppose also that the $\psi_2,
\psi_3, \ldots, \psi_J$ that define the corresponding joint manifold
$\manifold^*$ are diffeomorphisms.  If $1/\tau^*$ is the condition
number of $\manifold^*$, then
$$
\tau^* \ge \mathop{\min}_{1\le j \le J} \tau_j,
$$
or equivalently,
$$
\frac{1}{\tau^*} \le \mathop{\max}_{1 \le j \le J} \frac{1}{\tau_j}.
$$
\end{thm}
\begin{proof}
Let $p \in \manifold^*$, which we can write as $p = (p_1, p_2,
\ldots, p_J)$ with $p_j \in \manifold_j$. Since the
$\{\psi_j\}_{j=2}^J$ are diffeomorphisms, we may view $\manifold^*$
as being diffeomorphic to $\manifold_1$; i.e., we can build a
diffeomorphic map from $\manifold_1$ to $\manifold^*$ as
$$
p = \psi^*(p_1) := (p_1, \psi_2(p_2), \ldots, \psi_J(p_J)).
$$

We also know that given any two manifolds linked by a diffeomorphism
$\psi_j: \manifold_1 \to \manifold_j$, each vector $v_1$ in the
tangent space $T_1(p_1)$ of the manifold $\manifold_1$ at the point
$p_1$ is {\em uniquely} mapped to a tangent vector $v_j :=
\phi_j(v_1)$ in the tangent space $T_j(p_j)$ of the manifold
$\manifold_j$ at the point $p_j = \psi_j(p_1)$ through the map
$\phi_j := \jacobian \circ \psi_j(p_1)$ , where $\jacobian$ denotes
the Jacobian operator.

Consider the application of this property to the diffeomorphic manifolds $\manifold_1$ and $\manifold^*$. In this case, the tangent vector $v_1 \in T_1(p_1)$ to the manifold $\manifold_1$ can be uniquely identified with a tangent vector $v = \phi^*(v_1) \in T^*(p)$ to the manifold $\manifold^*$. This mapping is expressed as
\begin{equation}
\phi^*(v_1) = \jacobian \circ \psi^*(p_1) =  (v_1, \jacobian \circ
\psi_2(p_1), \ldots, \jacobian \circ \psi_J(p_1)), \nonumber
\end{equation}
since the Jacobian operates componentwise. Therefore, the tangent vector $v$ can be written as
\begin{eqnarray}
v &=& \phi^*(v_1) = (v_1, \phi_2(v_1), \ldots, \phi_J(p_1)), \nonumber \\
&=& (v_1, v_2, \ldots, v_J).
\nonumber
\end{eqnarray}
In other words, a tangent vector to the joint manifold can be decomposed into $J$ component vectors, each of which are tangent to the corresponding component manifolds.

Using this fact, we now show that a vector $\eta$ that is normal to
$\manifold^*$ can also be broken down into sub-vectors that are
normal to the component manifolds. Consider $p \in \manifold^*$, and
denote $T^*(p)^\perp$ as the normal space at $p$. Suppose $\eta =
(\eta_1, \ldots, \eta_J) \in T^*(p)^\perp$. Decompose each $\eta_j$
as a projection onto the component tangent and normal spaces, i.e.,
for $j = 1,\ldots, J$,
$$
\eta_j = x_j + y_j, \qquad x_j \in T_j(p_j),~y_j \in T_j(p_j)^\perp .
$$
such that $\iprod{x_j}{y_j} = 0$ for each $j$. Let $x = (x_1,
\ldots, x_J)$ and $y = (y_1, \ldots, y_J)$. Then $\eta = x+y$, and
since $y$ is tangent to the joint manifold $\manifold^*$, we have
$\iprod{\eta}{y} = \iprod{x+y}{x} = 0$, and thus
$$
\iprod{y}{x}=-\|x\|^2.
$$
But,
$$
\iprod{y}{x} = \sum_{j=1}^J \iprod{y_j}{x_j} = 0 .
$$
Hence $x = 0$, i.e., each $\eta_j$ is normal to $\manifold_j$.

Armed with this last fact, our goal now is to show that if $r < \min_{1 \le j \le J} \tau_j$ then the normal
bundle of radius $r$ is embedded in $\reals^\dim$, or equivalently,
that $p + \eta \neq q + \nu$ provided that $\|\eta\|, \|\nu\| \le
r$. Indeed, suppose $\|\eta\|, \|\nu\| \le r < \min_{1\le j \le J} \tau_j$. Since
$\|\eta_j\| \le \|\eta\|$ and $\|\nu_j\| \le \|\nu\|$ for all $1 \le j \le J$,
we have that $\|\eta_j\|, \|\nu_j\| < \min_{1 \le i \le J} \tau_i \le \tau_j$. Since we have proved that $\eta_j, \nu_j$ are vectors in the normal bundle of $\manifold_j$ and their magnitudes are less than $\tau_j$, then $p_j + \eta_j \neq q_j + \nu_j$ by the definition of condition number. Thus $p + \eta \neq q + \nu$ and the result follows.
\end{proof}

This result states that for general manifolds, the most we can say
is that the condition number of the joint manifold is guaranteed to
be less than that of the {\em worst} manifold.  However, in practice
this is not likely to happen.  As an example, Figure
\ref{fig:normal_bundle} illustrates the point at which the normal
bundle intersects itself for the case of the joint manifold from
Figure \ref{fig:helix} (c).  In this case we obtain $\tau^*
= \sqrt{\pi^2/2 + 1}$.  Note that the condition numbers for the
manifolds $\manifold_1$ and $\manifold_2$ generating $\manifold^*$
are given by $\tau_1 = \infty$ and $\tau_2 = 1$.  Thus, while the
condition number in this case is not as good as the best manifold,
it is still notably better than the worst manifold.  In general,
even this example may be somewhat pessimistic, and it is possible
that in many cases the joint manifold may be better conditioned than
even the best manifold.

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\hsize, viewport=50 60 400 300]{Figs/normal_bundle2}
\caption{\small\sl Point at which the normal bundle for the helix
manifold intersects itself.} \label{fig:normal_bundle}
\end{figure}

